Sketch2NeRF: Multi-view Sketch-guided Text-to-3D Generation

Recently, text-to-3D approaches have achieved high-fidelity 3D content generation using text description. However, the generated objects are stochastic and lack fine-grained control. Sketches provide a cheap approach to introduce such fine-grained control. Nevertheless, it is challenging to achieve flexible control from these sketches due to their abstraction and ambiguity. In this paper, we present a multi-view sketch-guided text-to-3D generation framework (namely, Sketch2NeRF) to add sketch control to 3D generation. Specifically, our method leverages pretrained 2D diffusion models (e.g., Stable Diffusion and ControlNet) to supervise the optimization of a 3D scene represented by a neural radiance field (NeRF). We propose a novel synchronized generation and reconstruction method to effectively optimize the NeRF. In the experiments, we collected two kinds of multi-view sketch datasets to evaluate the proposed method. We demonstrate that our method can synthesize 3D consistent contents with fine-grained sketch control while being high-fidelity to text prompts. Extensive results show that our method achieves state-of-the-art performance in terms of sketch similarity and text alignment.

==> figure/fig_results_prompt_variation.tex <==
\begin{figure}[t]
    \centering
    \begin{subfigure}{\linewidth}
        \includegraphics[width=0.32\linewidth]{image/results_prompt_variation/chair_sketch/r_114.png}
        \includegraphics[width=0.32\linewidth]{image/results_prompt_variation/chair_sketch/r_140.png}
        \includegraphics[width=0.32\linewidth]{image/results_prompt_variation/chair_sketch/r_55.png}
        \caption*{Sketch}
    \end{subfigure}
    \begin{subfigure}{\linewidth}
        \includegraphics[width=0.32\linewidth]{image/results_prompt_variation/a_chair_with_red_color/45_cropped.png}
        \includegraphics[width=0.32\linewidth]{image/results_prompt_variation/a_chair_with_red_color/75_cropped.png}
        \includegraphics[width=0.32\linewidth]{image/results_prompt_variation/a_chair_with_red_color/97_cropped.png}
        \caption*{Prompt: “\textit{A Chair with Red Color}”}
    \end{subfigure}
    \begin{subfigure}{\linewidth}
        \includegraphics[width=0.32\linewidth]{image/results_prompt_variation/a_chair_with_a_green_cushion/45_cropped.png}
        \includegraphics[width=0.32\linewidth]{image/results_prompt_variation/a_chair_with_a_green_cushion/75_cropped.png}
        \includegraphics[width=0.32\linewidth]{image/results_prompt_variation/a_chair_with_a_green_cushion/97_cropped.png}
        \caption*{Prompt: “\textit{A Chair with a Green Cushion}”}
    \end{subfigure}
    \caption{
        3D models generated with different prompts. 
    }
    \label{fig-results-prompt-variation}
    \vspace{0.0cm}
\end{figure}

==> figure/fig_suppl_additional_results.tex <==
\begin{figure*}[hbpt]
    \centering
    \begin{subfigure}{0.92\linewidth}
        \begin{minipage}[t]{\linewidth}
            \includegraphics[width=\linewidth]{image/suppl_additional_results/suppl_additional_results.jpg}
        \end{minipage}
    \end{subfigure}
    \caption{
        Additional visual results. \textit{Left}: input sketches. \textit{Right}: rendered images of generated 3D objects from our method.
    }
    \label{fig:suppl-additional-results}
    \vspace{-0.4cm}
\end{figure*}

==> figure/fig_suppl_comparison_with_single_sketch.tex <==
\begin{figure*}[hbpt]
    \centering
    \begin{subfigure}{0.12\linewidth}
        \begin{minipage}[t]{\linewidth}
            \includegraphics[width=\linewidth]{image/results_qualitative_comparisons/teddy_bear_001_sketch.jpg}
        \end{minipage}
        \caption*{Input Sketch}
    \end{subfigure}
    \begin{subfigure}{0.12\linewidth}
        \begin{minipage}[t]{\linewidth}
            \includegraphics[width=\linewidth]{image/results_qualitative_comparisons/teddy_bear_001_ours.jpg}
        \end{minipage}
        \caption*{Ours}
    \end{subfigure}
    \begin{subfigure}{0.12\linewidth}
        \begin{minipage}[t]{\linewidth}
            \includegraphics[width=\linewidth]{image/results_qualitative_comparisons/teddy_bear_001_zero123_controlnet.jpg}
        \end{minipage}
        \caption*{C-Zero123}
    \end{subfigure}
    \begin{subfigure}{0.12\linewidth}
        \begin{minipage}[t]{\linewidth}
            \includegraphics[width=\linewidth]{image/results_qualitative_comparisons/teddy_bear_001_magic123_controlnet.jpg}
        \end{minipage}
        \caption*{C-Magic123}
    \end{subfigure}
    \begin{subfigure}{0.12\linewidth}
        \begin{minipage}[t]{\linewidth}
            \includegraphics[width=\linewidth]{image/results_qualitative_comparisons/backpack_001_sketch.jpg}
        \end{minipage}
        \caption*{Input Sketch}
    \end{subfigure}
    \begin{subfigure}{0.12\linewidth}
        \begin{minipage}[t]{\linewidth}
            \includegraphics[width=\linewidth]{image/results_qualitative_comparisons/backpack_001_ours.jpg}
        \end{minipage}
        \caption*{Ours}
    \end{subfigure}
    \begin{subfigure}{0.12\linewidth}
        \begin{minipage}[t]{\linewidth}
            \includegraphics[width=\linewidth]{image/results_qualitative_comparisons/backpack_001_zero123_controlnet.jpg}
        \end{minipage}
        \caption*{C-Zero123}
    \end{subfigure}
    \begin{subfigure}{0.12\linewidth}
        \begin{minipage}[t]{\linewidth}
            \includegraphics[width=\linewidth]{image/results_qualitative_comparisons/backpack_001_magic123_controlnet.jpg}
        \end{minipage}
        \caption*{C-Magic123}
    \end{subfigure}
    \caption{
        Qualitative comparisons on 3 different objects with two single-sketch 3D generation approaches.
        Results clearly indicate that our method produces better consistent and high-fidelity 3D objects with multi-view sketch control.
    }
    \label{fig:suppl-comparisons-with-single-sketch}
    \vspace{-0.4cm}
\end{figure*}

==> table/tab_3d_consistency.tex <==
\begin{table}[htbp]
  \centering
  \caption{Quantitative comparisons of 3D Consistency on the OmniObject-Sketch dataset. (Note that we use the AlexNet~\cite{krizhevsky2012imagenet} as the backbone in LPIPS computation)}
    \resizebox{0.48\textwidth}{!}{
    \setlength{\tabcolsep}{1mm}{
        \begin{tabular}{l|cc|cc}
        \toprule
        \multirow{2}[2]{*}{} & \multicolumn{2}{c|}{Short-range} & \multicolumn{2}{c}{Long-range} \\
              & RMSE$\downarrow$  & LPIPS$\downarrow$ & RMSE$\downarrow$  & LPIPS$\downarrow$ \\
        \midrule
        DreamFusion~\cite{poole2022dreamfusion}         & 0.0790            & 0.0546            & 0.3426            & 0.2133 \\
        ProlificDreamer~\cite{wang2023prolificdreamer}  & 0.1453            & 0.0564            & 0.2104            & 0.1103 \\
        C-DreamFusion                                   & 0.1159            & 0.0928            & 0.3066            & 0.2396 \\
        C-ProlificDreamer                               & 0.5707            & 0.3742            & 0.6606            & 0.4536 \\
        Sketch2NeRF (Ours)                              & \textbf{0.0161}   & \textbf{0.0119}   & \textbf{0.0684}   & \textbf{0.0683} \\
        \bottomrule
        \end{tabular}%
    }}
    \vspace{-0.4cm}
  \label{tab:consistency_omniobject3d_sketch}%
\end{table}%

